Networked oscillator based modeling and control of unsteady wakes

A networked oscillator based analysis is performed for periodic bluff body flows to examine and control the transfer of kinetic energy. Spatial modes extracted from the flow field with corresponding amplitudes form a set of oscillators describing unsteady fluctuations. These oscillators are connected through a network that captures the energy exchanges amongst them. To extract the network of interactions among oscillators, amplitude and phase perturbations are impulsively introduced to the oscillators and the ensuing dynamics are analyzed. Using linear regression techniques, a networked oscillator model is constructed that reveals energy transfers and phase interactions among the modes. The model captures the nonlinear interactions amongst the modal oscillators through a linear approximation. A large collection of system responses are aggregated into a network model that captures interactions for general perturbations. The networked oscillator model describes the modal perturbation dynamics better than the empirical Galerkin reduced-order models. A model-based feedback controller is then designed to suppress modal amplitudes and the resulting wake unsteadiness leading to drag reduction. The strength of the proposed approach is demonstrated for a canonical example of two- dimensional unsteady flow over a circular cylinder. The present formulation enables the characterization of modal interactions to control fundamental energy transfers in unsteady vortical flows.

==> preamb.tex <==
\usepackage{graphicx}
\usepackage{natbib,color}
\usepackage{float}
\usepackage{amsmath,amssymb,stmaryrd,array} 
\usepackage{epsfig,color,soul,rotating,overpic}
\usepackage{subfig, setspace}
\usepackage{epstopdf}
\usepackage[section]{placeins}
\usepackage{float}
\usepackage{array}

% See if the author has AMS Euler fonts installed: If they have, attempt
% to use the 'upmath' package to provide upright math.
\ifCUPmtlplainloaded \else
  \checkfont{eurm10}
  \iffontfound
    \IfFileExists{upmath.sty}
      {\typeout{^^JFound AMS Euler Roman fonts on the system,
                   using the 'upmath' package.^^J}%
       \usepackage{upmath}}
      {\typeout{^^JFound AMS Euler Roman fonts on the system, but you
                   dont seem to have the}%
       \typeout{'upmath' package installed. JFM.cls can take advantage
                 of these fonts,^^Jif you use 'upmath' package.^^J}%
       \providecommand\upi{\pi}%
      }
  \else
    \providecommand\upi{\pi}%
  \fi
\fi

% See if the author has AMS symbol fonts installed: If they have, attempt
% to use the 'amssymb' package to provide the AMS symbol characters.

\ifCUPmtlplainloaded \else
  \checkfont{msam10}
  \iffontfound
    \IfFileExists{amssymb.sty}
      {\typeout{^^JFound AMS Symbol fonts on the system, using the
                'amssymb' package.^^J}%
       \usepackage{amssymb}%
       \let\le=\leqslant  \let\leq=\leqslant
       \let\ge=\geqslant  \let\geq=\geqslant
      }{}
  \fi
\fi

% See if the author has the AMS 'amsbsy' package installed: If they have,
% use it to provide better bold math support (with \boldsymbol).

\ifCUPmtlplainloaded \else
  \IfFileExists{amsbsy.sty}
    {\typeout{^^JFound the 'amsbsy' package on the system, using it.^^J}%
     \usepackage{amsbsy}}
    {\providecommand\boldsymbol[1]{\mbox{\boldmath $##1$}}}
\fi

% array strut to make delimiters come out right size both ends
\newsavebox{\astrutbox}
\sbox{\astrutbox}{\rule[-5pt]{0pt}{20pt}}
\newcommand{\astrut}{\usebox{\astrutbox}}

\newcommand\etal{\mbox{\textit{et al.}}}
\newcommand\etc{etc.\ }
\newcommand\eg{e.g.\ }
\newcommand\fig{figure }

\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

\newcommand\note[1]{\mbox{}\marginpar{\scriptsize\raggedright\hspace{0pt}\color{red}{#1}}}


